ECGtizer: a fully automated digitizing and signal recovery pipeline for electrocardiograms

Electrocardiograms (ECGs) are essential for diagnosing cardiac pathologies, yet traditional paper-based ECG storage poses significant challenges for automated analysis. This study introduces ECGtizer, an open-source, fully automated tool designed to digitize paper ECGs and recover signals lost during storage. ECGtizer facilitates automated analyses using modern AI methods. It employs automated lead detection, three pixel-based signal extraction algorithms, and a deep learning-based signal reconstruction module. We evaluated ECGtizer on two datasets: a real-life cohort from the COVID-19 pandemic (JOCOVID) and a publicly available dataset (PTB-XL). Performance was compared with two existing methods: the fully automated ECGminer and the semi-automated PaperECG, which requires human intervention. ECGtizer's performance was assessed in terms of signal recovery and the fidelity of clinically relevant feature measurement. Additionally, we tested these tools on a third dataset (GENEREPOL) for downstream AI tasks. Results show that ECGtizer outperforms existing tools, with its ECGtizerFrag algorithm delivering superior signal recovery. While PaperECG demonstrated better outcomes than ECGminer, it required human input. ECGtizer enhances the usability of historical ECG data and supports advanced AI-based diagnostic methods, making it a valuable addition to the field of AI in ECG analysis.

==> Chapter/Pipeline_ECGtizer.tex <==
\begin{figure*}[htbp] % Placement de l'image
    \centering
    %\FloatBarrier
    \includegraphics[width=\textwidth]{image/pipelineECGtizer.png} 
    \caption{\textbf{Figure from the ECGtizer pipeline.}First, the paper ECG is converted into an RGB matrix from the scanned image. Next, the text contained in the image is extracted and saved in a separate table, and the text is removed from the image. Once the text has been isolated, the positions of the ECG traces are detected in the matrix. Finally, once the traces have been isolated, they are extracted, cut into individual leads and scaled.}
    \label{fig:Pipeline}
\end{figure*}

==> tables/Table_Delta_Peak_With_PaperECG.tex <==
\begin{table*}[t]
    \centering
    \caption{$\Delta$ QT and $\Delta$ QRS represent the differences in segment lengths (in seconds), while $\Delta$ X$_{\text{amp}}$ represents the difference in peak amplitude (in mV) between the digitized and original signal (before lead-completion phase).}
    \begin{tabular}{l |c|c||c|c|c|c|c}
& $\Delta$QT  & $\Delta$QRS  & $\Delta$ R$_{\text{amp}}$  & $\Delta$ P$_{\text{amp}}$   & $\Delta$ Q$_{\text{amp}}$  & $\Delta$ S$_{\text{amp}}$  & $\Delta$ T$_{\text{amp}}$  \\
\midrule

{\ecgminer} & \textbf{0.001}±0.11  & \textbf{0.003}±0.04  & \textbf{-0.011}±0.42  & 0.685±0.52 & 0.783±0.56  & 0.877±0.60 & 0.657±0.46\\

{\paperecg} & \textbf{0.001}±0.08  & \textbf{0.003}±0.02  & -0.548±0.43 & -0.056±0.16 & 0.111±0.21  & 0.132±0.19 & -0.097±0.10\\  

{\ecgtizer}$_{\text{Full}}$       & 0.002±0.08  & 0.004±0.02  & -0.080±0.24 & -0.007±0.16 & \textbf{0.027}±0.22  &\textbf{0.023}±0.16 & -0.002±0.09 \\

{\ecgtizer}$_{\text{Frag}}$ & -0.005±0.14 & -0.005±0.08     & -0.074±0.11 & \textbf{0.000}±0.15 & 0.070±0.33  & 0.062±0.27 & \textbf{-0.001}±0.2 \\

{\ecgtizer}$_{\text{Lazy}}$       & 0.003±0.14  & 0.016±0.06  & 0.778±0.95  & 0.029±0.23 & -0.200±0.34  & -0.280±0.43 & 0.124±0.22 



\end{tabular}
\label{tab:Performance_method_with_PaperECG}
\end{table*}

==> tables/Table_Delta_Peak_With_PaperECG_comp.tex <==
\begin{table*}[t]
    \centering
    \caption{$\Delta$ QT and $\Delta$ QRS represent the differences in segment lengths (in seconds), while $\Delta$ X$_{\text{amp}}$ represents the difference in peak amplitude (in mV) between the digitized original signal (after lead-completion phase with {\ecgrecover}).}
    \begin{tabular}{l| c|c||c|c|c|c|c}
& $\Delta$QT  & $\Delta$QRS  & $\Delta$ R$_{\text{amp}}$  & $\Delta$ P$_{\text{amp}}$   & $\Delta$ Q$_{\text{amp}}$  & $\Delta$ S$_{\text{amp}}$  & $\Delta$ T$_{\text{amp}}$\\

\midrule

{\ecgminer} & -0.029±0.08 & -0.010±0.03 & -0.506± 0.42 & \textbf{-0.047}±0.05 & 0.117±0.13 & 0.153±0.16 & -0.113±0.08 \\

{\paperecg} &\textbf{0.000}±0.08 & 0.002±0.02 & -0.467±0.38 & -0.054±0.05 & 0.093±0.13  & 0.126±0.15 & -0.104±0.07  \\

{\ecgtizer}$_{\text{Full}}$ & \textbf{0.000}±0.08 & -0.002±0.02 & \textbf{-0.007}±0.13
 & -0.088±0.06 & -0.039±0.14  & \textbf{-0.010}±0.11 & -0.041±0.07  \\

{\ecgtizer}$_{\text{Frag}}$ &\textbf{0.000}±0.08  & \textbf{0.000}±0.02  & -0.016±0.15 & -0.088±0.07 & \textbf{-0.029}±0.15 & -0.012±0.12 & \textbf{-0.037}±0.07  \\

{\ecgtizer}$_{\text{Lazy}}$ &\textbf{0.000}±0.08  & 0.002±0.02 & 0.834±0.87 & -0.145±0.13 & -0.330±0.27 & -0.375±0.30 & 0.086±0.18 
\end{tabular}
\label{tab:Performance_method_comp_with_PaperECG_after}
\end{table*}

==> tables/table1.tex <==
\begin{table}[]
    \centering
    \caption{Performance of the {\ecgrecover} model in terms of PCC in reconstructing ECGs digitized with {\ecgtizer} (Metacardis) and comparison with its performance on the Generepol dataset as reported in the original paper~\cite{}.\textcolor{red}{35. Standard deviation? }}
    \begin{tabular}{r|c|c}
    \toprule
        Lead & {\ecgrecover} & {\ecgtizer}+{\ecgrecover}   \\
                \midrule                
                \textbf{I}   & \textbf{0.82} & \textbf{0.82} \\
                \textbf{II}  & \textbf{0.9} & 0.85 \\
                \textbf{III} & 0.54 & \textbf{0.55}  \\
                \textbf{aVL} & 0.69 & \textbf{0.71}  \\
                \textbf{aVR} & \textbf{0.92} & 0.85 \\
                \textbf{aVF} & \textbf{0.78} & 0.66 \\
                \textbf{V1}  & \textbf{0.87} & \textbf{0.87} \\
                \textbf{V2}  & \textbf{0.88} & 0.82 \\
                \textbf{V3}  & \textbf{0.84} & 0.78 \\
                \textbf{V4}  & \textbf{0.90} & 0.78 \\
                \textbf{V5}  & \textbf{0.93} & 0.84 \\
                \textbf{V6}  & \textbf{0.95} & 0.88\\
    \bottomrule
    \end{tabular}
    \label{tab:PCC_recover}
\end{table}

\begin{table}[]
    \centering
    \caption{Performance of the {\ecgrecover} model in terms of RMSE in reconstructing ECGs digitized with {\ecgtizer} (Metacardis) and comparison with its performance on the Generepol dataset as reported in the original paper~\cite{}.}
    \begin{tabular}{r|c|c}
    \toprule
        Lead & {\ecgrecover} & {\ecgtizer}+{\ecgrecover}   \\
                \midrule 
                              \textbf{I}   & 0.20 & \textbf{0.12} \\
                \textbf{II}  & 0.14 & \textbf{0.08} \\
                \textbf{III} & 0.32 & \textbf{0.12}  \\
                \textbf{aVL} & 0.29 & \textbf{0.10}  \\
                \textbf{aVR} & 0.14 & \textbf{0.08} \\
                \textbf{aVF} & 0.20 & \textbf{0.08} \\
                \textbf{V1}  & 0.18 & \textbf{0.07} \\
                \textbf{V2}  & 0.17 & \textbf{0.12} \\
                \textbf{V3}  & 0.23 & \textbf{0.20} \\
                \textbf{V4}  & \textbf{0.15} & 0.22 \\
                \textbf{V5}  & \textbf{0.12} & 0.13 \\
                \textbf{V6}  & 0.11 & \textbf{0.09}\\
                \bottomrule
    \end{tabular}
    \label{tab:RMSE_recover}
\end{table}

\begin{table}[]
       \centering
    \caption{Performance of the {\ecgrecover} model in terms of STDW in reconstructing ECGs digitized with {\ecgtizer} (Metacardis) and comparison with its performance on the Generepol dataset as reported in the original paper~\cite{}.}
    \begin{tabular}{r|c|c}
    \toprule
        Lead & {\ecgrecover} & {\ecgtizer}+{\ecgrecover}   \\
                \midrule 
                \textbf{I}   & \textbf{0.04} & 0.05 \\
                \textbf{II}  & \textbf{0.02} & 0.03 \\
                \textbf{III} & 0.10 & \textbf{0.06 } \\
                \textbf{aVL} & 0.08 & \textbf{0.04}  \\
                \textbf{aVR} & \textbf{0.02} & 0.03 \\
                \textbf{aVF} & 0.04 & \textbf{0.03} \\
                \textbf{V1}  & \textbf{0.03} & \textbf{0.03} \\
                \textbf{V2}  & \textbf{0.03} & 0.06 \\
                \textbf{V3}  & \textbf{0.05} & 0.16 \\
                \textbf{V4}  & \textbf{0.02} & 0.19 \\
                \textbf{V5}  & \textbf{0.02} & 0.07 \\
                \textbf{V6}  & \textbf{0.01} & 0.07\\
                \hline
    \end{tabular}
    \label{tab:STDW_recover}
\end{table}


==> tables/table2.tex <==

\begin{table}[]
    \centering
    \caption{Difference in seconds (s) and in millivolts (mV) between the positions of the peaks in the original ECGs and their digitized counterparts. }
    \begin{tabular}{r|c|c}
                \toprule
                 & {\ecgtizer} & {\ecgminer} \\
                \midrule
                $\Delta$P ($\mu$sec) & \textbf{2.94} ± 28.72 & 3.53 ± 42.77 \\
                $\Delta$Q ($\mu$sec) & \textbf{8.96} ± 15.81 & 10.57 ± 19.83 \\
                $\Delta$R ($\mu$sec) & \textbf{0} ± 0 & \textbf{0} ± 0 \\
                $\Delta$S ($\mu$sec) & \textbf{11.96} ± 31.56 & 14.93 ± 43.07 \\
                $\Delta$T ($\mu$sec) & 13.14 ± 64.92 & \textbf{11.62} ± 101.34 \\
                \midrule
                $\Delta$P (mV) & \textbf{0.02} ± 0.04 & 0.35 ± 1.59 \\
                $\Delta$Q (mV) & \textbf{0.02} ± 0.05 & 0.33 ± 1.22 \\
                $\Delta$R (mV) & \textbf{0.14} ± 0.08 & 0.18 ± 1.52 \\
                $\Delta$S (mV) & \textbf{0.0} ± 0.13 & 0.31 ± 1.25 \\
                $\Delta$T (mV) & \textbf{0.02} ± 0.03 & 0.33 ± 1.55 \\
                \bottomrule
    \end{tabular}
    \label{tab:amp_sec_comp_table}
    % \label{tab:my_label}
\end{table}
